Calculated attributes of synonym sets

The goal of formalization, proposed in this paper, is to bring together, as near as possible, the theoretic linguistic problem of synonym conception and the computer linguistic methods based generally on empirical intuitive unjustified factors. Using the word vector representation we have proposed the geometric approach to mathematical modeling of synonym set (synset). The word embedding is based on the neural networks (Skip-gram, CBOW), developed and realized as word2vec program by T. Mikolov. The standard cosine similarity is used as the distance between word-vectors. Several geometric characteristics of the synset words are introduced: the interior of synset, the synset word rank and centrality. These notions are intended to select the most significant synset words, i.e. the words which senses are the nearest to the sense of a synset. Some experiments with proposed notions, based on RusVectores resources, are represented. A brief description of this work can be viewed in slides https://goo.gl/K82Fei

==> chapter/biblio.bib_check_addons.tex <==
@book{AlexandrovaSynDict_2001,
 author = {Alexandrova~Z.~E.},
 title = {{Slovar' sinonimov ruskogo jazyka [Russian dictionary of synonyms]}},
 publisher = {Russkij jazyk [Russian language]},
 year = {2001},
 address = {Moscow},
 pagetotal = {586}
}
// Александрова З.Е. Словарь синонимов руского языка // М. Русский язык. 2001 г. 568 с.


// Баранов В.И.,Стечкин Б.С. Экстремальные комбинаторные задачи и их приложения. М.: Физматлит. ISBN: 5-9221-0493-4. 2004. 238 с. (с. 24). 
@book{Baranov_Stechkin_2004,
 author = {Baranov~V.~I., Stechkin~B.~S.},
 title = {{Jekstremal'nye kombinatornye zadachi i ih prilozhenija [Extreme combinatorial problems and their applications]}},
 publisher = {Fizmatlit [FIZMATLIT]},
 year = {2004},
 address = {Moscow},
 pagetotal = {238}
 ISBN = {5-9221-0493-4},
}


@article{Kaushinis_2015,
  author = {T. V. Kaushinis and A. N. Kirillov and N. I. Korzhitsky and A. A. Krizhanovsky and A. V. Pilinovich and I. A. Sikhonina and A. M. Spirkova and V. G. Starkova and T. V. Stepkina and S. S. Tkach and Ju. V. Chirkova and A. L. Chuharev and D. S. Shorets and D. Yu. Yankevich and E. A. Yaryshkina},
  title = {{A review of word-sense disambiguation methods and algorithms: Introduction}},
  number = {2},
  doi = {10.17076/mat135},
  number = {10},
  journal = {Transactions of Karelian Research Centre of Russian Academy of Science},
  series = {Mathematical Modeling and Information Technologies},
  year = {2015},
  pages={69--98},
  url = {\url{http://journals.krc.karelia.ru/index.php/mathem/article/view/135}},
}


@article{Goldberg_2014_word2vec,
  title={word2vec explained: Deriving mikolov et al.'s negative-sampling word-embedding method},
  author={Goldberg, Yoav and Levy, Omer},
  journal={arXiv preprint arXiv:1402.3722},
  pages={1--5},
  year={2014}
}


% Ronald L. Graham, Donald E. Knuth, Oren Patashnik (1988) Concrete Mathematics, Addison–Wesley, Reading MA. ISBN 0-201-14236-8, p. 244.
@book{graham1994concrete,
  title={Concrete mathematics},
  author={Ronald L. Graham, Donald E. Knuth, Oren Patashnik},
  year={1994},
  publisher={Addison–Wesley},
  ISBN={0-201-14236-8},
}


@inproceedings{Huang_2012,
 author = {Huang, Eric H. and Socher, Richard and Manning, Christopher D. and Ng, Andrew Y.},
 title = {{Improving Word Representations via Global Context and Multiple Word Prototypes}},
 booktitle = {Proceedings of the 50th Annual Meeting of the Association for Computational Linguistics},
 series = {ACL '12},
 year = {2012},
 location = {Jeju Island, Korea},
 pages = {873--882},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=2390524.2390645},
 acmid = {2390645},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
}


@article{Krizhanovsky_Smirnov_2013,
  author = {Krizhanovsky, Andrew and Smirnov, Alexander},
  title = {{An approach to automated construction of a general-purpose lexical ontology based on Wiktionary}},
  volume = {52},
  url = {http://scipeople.com/publication/113533/},
  doi = {10.1134/S1064230713020068},
  number = {2},
  journal = {Journal of Computer and Systems Sciences International},
  year = {2013},
  pages = {215-225},
}


@inproceedings{Kutuzov_2015,
  doi = {10.1007/978-3-319-18111-0_4},
  url = {https://www.academia.edu/11754162/Comparing_neural_lexical_models_of_a_classic_national_corpus_and_a_web_corpus_the_case_for_Russian},
  year = {2015},
  publisher = {Springer Science + Business Media},
  pages = {47--58},
  author = {Andrey Kutuzov and Elizaveta Kuzmenko},
  title = {{Comparing Neural Lexical Models of a Classic National Corpus and a Web Corpus: The Case for Russian}},
  booktitle = {Computational Linguistics and Intelligent Text Processing},
}


@article{Levy_2015_Improving,
  title={Improving distributional similarity with lessons learned from word embeddings},
  author={Levy, Omer and Goldberg, Yoav and Dagan, Ido},
  journal={Transactions of the Association for Computational Linguistics},
  volume={3},
  pages={211--225},
  year={2015}
}


@article{Mahadevan_2015_Reasoning,
  title={Reasoning about linguistic regularities in word embeddings using matrix manifolds},
  author={Mahadevan, Sridhar and Chandar, Sarath},
  journal={arXiv preprint arXiv:1507.07636},
  pages={1--9},
  year={2015}
}


@inproceedings{Mikolov_2011,
  doi = {10.1109/icassp.2011.5947611},
  url = {http://dx.doi.org/10.1109/icassp.2011.5947611},
  year = {2011},
  month = {may},
  publisher = {Institute of Electrical {\&} Electronics Engineers ({IEEE})},
  author = {Tomas Mikolov and Stefan Kombrink and Lukas Burget and Jan Cernocky and Sanjeev Khudanpur},
  title = {{Extensions of recurrent neural network language model}},
  booktitle = {2011 {IEEE} International Conference on Acoustics Speech and Signal Processing ({ICASSP})},
}


@inproceedings{Mikolov_2012,
  doi = {10.1109/slt.2012.6424228},
  url = {http://dx.doi.org/10.1109/slt.2012.6424228},
  year = {2012},
  month = {dec},
  publisher = {Institute of Electrical {\&} Electronics Engineers ({IEEE})},
  author = {Tomas Mikolov and Geoffrey Zweig},
  title = {{Context dependent recurrent neural network language model}},
  booktitle = {2012 {IEEE} Spoken Language Technology Workshop ({SLT})},
}


@article{Mikolov_2013,
  title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  journal={arXiv preprint arXiv:1301.3781},
  year={2013}
  url = {http://arxiv.org/abs/1301.3781},
}


@inproceedings{rehurek_lrec,
      title = {{Software Framework for Topic Modelling with Large Corpora}},
      author = {Radim {\v R}eh{\r u}{\v r}ek and Petr Sojka},
      booktitle = {{Proceedings of the LREC 2010 Workshop on New
           Challenges for NLP Frameworks}},
      pages = {45--50},
      year = 2010,
      month = May,
      day = 22,
      publisher = {ELRA},
      address = {Valletta, Malta},
      note={\url{http://is.muni.cz/publication/884893/en}},
      language={English}
}



@misc{WordNet,
  author = {{Princeton University}},
  title = {{About WordNet}},
  year = {2016},
  howpublished = {\url{http://wordnet.princeton.edu}},
  note = {Online; accessed 30-April-2016}
}


@article{Sidorov_2014_Soft,
  title={Soft similarity and soft cosine measure: Similarity of features in vector space model},
  author={Sidorov, Grigori and Gelbukh, Alexander and G{\'o}mez-Adorno, Helena and Pinto, David},
  journal={Computaci{\'o}n y Sistemas},
  volume={18},
  number={3},
  pages={491--504},
  year={2014},
  publisher={Centro de Investigaci{\'o}n en Computaci{\'o}n, IPN},
  url={http://www.scielo.org.mx/pdf/cys/v18n3/v18n3a7.pdf}
}
